A Forensic Audit of the Tor Browser Bundle

The increasing use of encrypted data within file storage and in network communications leaves investigators with many challenges. One of the most challenging is the Tor protocol, as its main focus is to protect the privacy of the user, in both its local footprint within a host and over a network connection. The Tor browser, though, can leave behind digital artefacts which can be used by an investigator. This paper outlines an experimental methodology and provides results for evidence trails which can be used within real-life investigations.

==> 1.tex <==
Aggarwal et al. (2010). An Analysis of Private Browsing Modes in Modern Browsers.

Darcie, W et al. (2014). Online Anonymity: Forensic Analysis of the Tor Browser Bundle. 

David, A., \& Hargreaves, C. (2012). An analysis of Hotmail artefacts in Firefox. 6th Cybercrime Forensics Education and Training, 1–20.

Dayalamurthy, D. (2013). Forensic Memory Dump Analysis and Recovery of Artefacts of Using the Tor Browser Bundle – the Need

Dewey, C. (2013, October 3). The Switch. Everything we Know About Ross Ulbricht, the Outdoorsy Libertarian Behind Silk Road. Retrieved 22 March 2018 from https://www.washingtonpost.com/news/the-switch/wp/2013/10/03/everything-we-know-about-ross-ulbricht-the-outdoorsy-libertarian-behind-silk-road/?utm_term=.8e2751dccfd8

Epifani, M et al. (2014, March 24). Tor Forensics on Windows OS. 

Findlay, C \& Leimich, P. (2014, July). An Assessment of Data Leakage in Firefox Under Different Conditions. 

Gleeda. (2017). Volatility Foundation. Command Reference. Retrieved 22 March 2018 from https://github.com/volatilityfoundation/volatility/wiki/Command-Reference

Greenwald et al. (2013, June 11). The Guardian. Edward Snowden: the Whistleblower Behind the NSA Surveillance Revelations. Retrieved 01 April 2018 from https://www.theguardian.com/world/2013/jun/09/edward-snowden-nsa-whistleblower-surveillance

Montasari, R., \& Peltola, P. (2015, September). Computer forensic analysis of private browsing modes. In International Conference on Global Security, Safety, and Sustainability (pp. 96-109). Springer, Cham.

Noorulla, E. (2014, June 6). Web Browser Private Mode Forensic Analysis. 

Nordberg, L. (2016). The State of Academic Research in Tor

Perry et al. (2018, February 19). The Design and Implementation of the Tor Browser [DRAFT]. Retrieved 16 March 2018 from   https://www.torproject.org/projects/torbrowser/design/

Roussas, G. (2009, June 22). Vizuaxflisation of Client-Side Web Browsing and Email Activity

Sandvik, R. (2013, June 28). Forensic Analysis of the Tor Browser Bundle on OSX, Linux and Windows

Shepherd, E. (2017, July 17). The Places Database. Mozilla Developer Network Web Docs. Retrieved 5 January 2018 from https://developer.mozilla.org/en-US/docs/Mozilla/Tech/Places/Database

Support.mozilla.org. (2018). Private Browsing: Use Firefox Without Saving History. Retrieved 20 January 2018 from https://support.mozilla.org/en-US/kb/private-browsing-use-firefox-without-history?redirectlocale=en-US&redirectslug=private-browsing-browse-web-without-saving-info

Torproject.org. (2018a). Tor: Overview. Retrieved 01 April 2018 from https://www.torproject.org/about/overview.html.en

Tsalis et al. (2017). Exploring the Protection of Private Browsing in Desktop Browsers.

Warren, A. (2017, February 22). Tor Browser Artefacts in Windows 10.
